Problems in NP can Admit Double-Exponential Lower Bounds when Parameterized by Treewidth or Vertex Cover

Treewidth (tw) is an important parameter that, when bounded, yields tractability for many problems. For example, graph problems expressible in Monadic Second Order (MSO) logic and QUANTIFIED SAT or, more generally, QUANTIFIED CSP, are FPT parameterized by the tw of the input's (primal) graph plus the length of the MSO-formula [Courcelle, Information & Computation 1990] and the quantifier rank [Chen, ECAI 2004], resp. The algorithms from these (meta-)results have running times whose dependence on tw is a tower of exponents. A conditional lower bound by Fichte et al. [LICS 2020] shows that, for QUANTIFIED SAT, the height of this tower is equal to the number of quantifier alternations. Lower bounds showing that at least double-exponential factors in the running time are necessary are rare: there are very few (for tw and vertex cover vc parameterizations) and they are for problems that are complete for #NP, $\Sigma_2^p$, $\Pi_2^p$, or higher levels of the polynomial hierarchy. We show, for the first time, that it is not necessary to go higher up in the polynomial hierarchy to obtain such lower bounds. We design a novel, yet simple versatile technique based on Sperner families to obtain such lower bounds and apply it to 3 problems: METRIC DIMENSION, STRONG METRIC DIMENSION, and GEODETIC SET. We prove that they do not admit $2^{2^{o(tw)}} \cdot n^{O(1)}$-time algorithms, even on bounded diameter graphs, unless the ETH fails. For STRONG METRIC DIMENSION, the lower bound holds even for vc. We complement our lower bounds with matching upper bounds.

==> algo-tw-diam.tex <==
\section{Algorithms for Diameter plus Treewidth Parameterization}
\label{sec:algo-tw-diam-MD-GS}

The aim of this section is to prove the following theorem.
\begin{theorem}
\label{thm:algo-diam-tw}
\mdfull and \gsfull admit algorithms running in time
$2^{\diam^{\mathcal{O}(\tw)}} \cdot n^{\OO(1)}$.
\end{theorem}
To this end, we give a dynamic programming algorithm on a tree decomposition for each of these two problems. Both algorithms are inspired by the one from~\cite{BDP23} for chordal graphs, though there are some non-trivial differences. In each case, we will assume that a tree decomposition of the input graph $G$ of width $w$ is given to us. Note that one can compute a tree decomposition of width $w\leq 2\tw(G)+1$ in time $2^{\OO(\tw(G))}n$~\cite{K21}, and it can be transformed into a \emph{nice tree decomposition} of the same width with $\OO(wn)$ bags in time $\OO(w^2n)$~\cite{niceTW}.

\input{algo-diam-tw-MD}
\input{algo-tw-diam-GS}

==> algo-vc.tex <==
\section{Algorithms for Vertex Cover Parameterization}
\label{sec:algo-vc-MD-GS-SMD}
\begin{comment}

In the first two subsections of this section,
we prove the following theorem.

\begin{theorem}
\label{thm:algo-vertex-cover}
\mdfull and \gsfull admit
\begin{itemize}
\item \FPT\ algorithms running in time
$2^{\mathcal{O}(\vc^2)} \cdot n^{\OO(1)}$, and
\item kernelization algorithms that 
output kernels with $2^{\OO(\vc)}$ vertices.
\end{itemize}
\end{theorem}

%\begin{theorem}
%\label{thm:algo-vertex-cover}
%\mdfull and \gsfull admit
%\begin{itemize}
%\item \FPT\ algorithms running in time
%$2^{\mathcal{O}(\vc^2)} \cdot n^{\OO(1)}$, and
%\item kernelization algorithms that 
%output kernels with $2^{\OO(\vc)}$ vertices.
%\end{itemize}
%\end{theorem}
%
%\begin{theorem}
%\label{thm:smd-algo-vertex-cover}
%\smdfull admits 
%\begin{itemize}
%\item an \FPT\ algorithm running in time
%$2^{2^{\mathcal{O}(\vc)}} \cdot n^{\OO(1)}$, and
%\item a kernelization algorithm that outputs a kernel with
%  $2^{\OO(\vc)}$ vertices.
%\end{itemize}
%\end{theorem}

\input{algo-vertex-cover-MD}
\input{algo-vertex-cover-GS}
\end{comment}
\input{algo-vertex-cover-SMD}

==> algo-vertex-cover-GS.tex <==
%\section{\gsfull: Algorithms for Vertex Cover Parameterization}
\subsection{Algorithm for \gsfull}
\label{sec:algo-fpt-vertex-cover-GS}

To prove Theorem~\ref{thm:algo-vertex-cover} for \gsfull, we start with the following fact about false twins.

%We start with the following fact about \emph{simplicial vertices} (a vertex is simplicial if its neighborhood forms a clique) and \emph{false twins} (vertices are false twins if they share the same open neighborhood). 
%%
%% \begin{observation}\label{obs:simplicial}
%% If a graph $G$ contains a simplicial vertex $v$, then $v$ belongs to any geodetic set of $G$.
%% \end{observation}
%% \begin{proof}
%% Observe that $v$ does not belong to any shortest path between any pair $x,y$ of vertices (both distinct from $v$).
%% \end{proof}

\begin{lemma}\label{lemma:open-twins}
If a graph $G$ contains a set $T$ of false twins that are not true twins and not simplicial, then any minimum-size geodetic set contains at most four vertices of $T$.
\end{lemma}
\begin{proof}
  Let $T=\{t_1,\ldots,t_h\}$ be a set of false twins in a graph $G$, that are not true twins and not simplicial. Thus, $T$ forms an independent set, and there are two non-adjacent vertices $x,y$ in the neighborhood of the vertices in $T$. Assume by contradiction that $h\geq 5$ and $G$ has a minimum-size geodetic set $S$ that contains at least five vertices of $T$; without loss of generality, assume $\{t_1,\ldots, t_5\}\subseteq S$. We claim that $S'=(S\setminus\{t_1,t_2,t_3\})\cup\{x,y\}$ is still a geodetic set, contradicting the choice of $S$ as a minimum-size geodetic set of $G$.

  To see this, notice that any vertex from $V(G)\setminus T$ that is covered by some pair of vertices in $T\cap S$ is also covered by $t_4$ and $t_5$. Similarly, any vertex from $V(G)\setminus T$ covered by some pair $\langle t_i,z \rangle$ in $(S\cap T)\times (S\setminus T)$, is still covered by $t_4$ and $z$. Moreover, $x$ and $y$ cover all vertices of $T$, since they are at distance~2 from each other and all vertices in $T$ are their common neighbors. Thus, $S'$ is a geodetic set, as claimed.  
\end{proof}

\begin{lemma}
\label{lemma:kernel-vc-GS}
\gsfull, parameterized by the vertex cover number $\vc$, admits a polynomial-time kernelization algorithm that returns an instance with $2^{\OO(\vc)}$ vertices.
\end{lemma}
\begin{proof}
Given a graph $G$,  let $X\subseteq V(G)$ be a minimum-size vertex cover of $G$. 
If this vertex cover is not given, then we can find a $2$-factor approximate vertex cover in polynomial time.
Let $I:=V(G)\setminus X$; $I$ forms an independent set. The kernelization algorithm exhaustively applies the following reduction rules in a sequential manner.

\begin{reduction rule} 
\label{reduc:simplicial}
If there exist three simplicial vertices in $G$ that are false twins or true twins, then delete one of them from $G$ and decrease $k$ by one.
\end{reduction rule}


\begin{reduction rule} 
\label{reduc:open-twins}
If there exist six vertices in $G$ that are false twins but are not true twins nor simplicial, then delete one of them from $G$.
%If there exist five vertices in $G$ that are false twins but not simplicial, then delete one of them from $G$.
%\ftodo{can also be proved with 5 instead of 6, but proof becomes slightly longer}
\end{reduction rule}

To see that Reduction Rule~\ref{reduc:simplicial} is correct, assume that $G$ contains three simplicial vertices $u,v,w$ that are twins (false or true). We show that $G$ has a geodetic set of size $k$ if and only if the reduced graph $G'$, obtained from $G$ by deleting $u$, has a geodetic set of size $k-1$. For the forward direction, let $S$ be a geodetic set of $G$ of size $k$. By Observation~\ref{obs:simplicial}, $S$ contains each of $u,v,w$. Now, let $S'=S\setminus\{u\}$. This set of size $k-1$ is a geodetic set of $G'$. Indeed, any vertex of $G'$ that was covered in $G$ by $u$ and some other vertex $z$ of $S$, is also covered by $v$ and $z$ in $G'$. Conversely, if $G'$ has a geodetic set $S''$ of size $k-1$, then it is clear that $S''\cup\{u\}$ is a geodetic set of size $k$ in $G$.

For Reduction Rule~\ref{reduc:open-twins}, assume that $G$ contains six false twins (that are not true twins nor simplicial) as the set $T=\{t_1,\ldots,t_6\}$, and let $G'$ be the reduced graph obtained from $G$ by deleting $t_1$. We show that $G$ has a geodetic set of size $k$ if and only if $G'$ has a geodetic set of size $k$. For the forward direction, let $S$ be a minimum-size geodetic set of size (at most) $k$ of $G$. By Lemma~\ref{lemma:open-twins}, $S$ contains at most four vertices from $T$; without loss of generality, $t_1$ and $t_2$ do not belong to $S$. Since the distances among all pairs of vertices in $G'$ are the same as in $G$, $S$ is still a geodetic set of $G'$. Conversely, let $S'$ be a minimum-size geodetic set of $G'$ of size (at most) $k$. Again, by Lemma~\ref{lemma:open-twins}, we may assume that one vertex among $t_2,\ldots,t_6$ is not in $S'$, say, without loss of generality, that it is $t_2$. Note that $S'$ covers (in $G$) all vertices of $G'$. Thus, $t_2$ is covered by two vertices $x,y$ of $S'$. But then, $t_1$ is also covered by $x$ and $y$, since we can replace $t_2$ by $t_1$ in any shortest path between $x$ and $y$. Hence, $S'$ is also a geodetic set of $G$. 

%FF: PROOF FOR 5 INSTEAD OF 6
%For Reduction Rule~\ref{reduc:open-twins}, assume that $G$ contains five false twins as the set $T=\{t_1,\ldots,t_5\}$, and let $G'$ be the reduced graph obtained from $G$ by deleting $t_1$. We show that $G$ has a geodetic set of size $k$ if and only if $G'$ has a geodetic set of size $k$. Let $S$ be a geodetic set of size $k$ of $G$. By Lemma~\ref{lemma:open-twins}, $S$ contains at most four vertices among $T$; without loss of generality, $t_1$ does not belong to $S$. Since the distances among all pairs in $G'$ are the same as in $G$, $S$ is still a geodetic set of $G'$. Conversely, let $S$ be a geodetic set of $G'$ of size $k$. Similarly, $S'$ covers (in $G$) all vertices of $G'$. If $t_1$ is also covered, we are done. So, assume next that $t_1$ is not covered. If any other vertex in $\{t_2,\ldots,t_5\}$ is not in $G$ by $S'$, then it would also not be covered by $S'$ in $G'$, a contradiction. So, all of $t_2,\ldots,t_5$ are in $S'$. As in the proof of Lemma~\ref{lemma:open-twins}, let $x,y$ be two non-adjacent vertices in the neighborhood of $t_1$ (they exist since $t_1$ is not simplicial), and let $S''=S'\setminus\{t_2,t_3\}\cup\{x,y\}$. Notice that all vertices not in $T$ that were covered by one of $t_2,t_3$ and some $z$ are still covered by $t_4$ and $z$, and all vertices of $T$ are now covered by $x,y$. Thus, $S''$ is a geodetic set of size $k$ in $G$.

Now, consider an instance on which the reduction rules cannot be applied. If $k<0$, then we return a trivial \no-instance (for example, a single-vertex graph). Otherwise, notice that any set of false twins in $I$ contains at most five vertices. Hence, $G$ has at most $|X| + 5 \cdot 2^{|X|} = 2^{\OO(\vc)}$ vertices.
\end{proof}

Next, we present an \XP-algorithm parameterized by the vertex cover number. Together with Lemma~\ref{lemma:kernel-vc-GS}, they imply Theorem~\ref{thm:algo-vertex-cover} for \gsfull.

\begin{lemma}
\label{lemma:algo-xp-vc-GS}
\gsfull admits an algorithm running in time $n^{\calO(\vc)}$.
\end{lemma}
\begin{proof}
The algorithm starts by computing a minimum vertex cover $X$ of $G$ in time $2^{\mathcal{O}(\vc)} \cdot n^{\calO(1)}$ using an \FPT\ algorithm for the \textsc{Vertex Cover} problem, for example the one in~\cite{DBLP:journals/jal/ChenKJ01}. Let $I := V(G)\setminus X$.

In polynomial time, we compute the set $S$ of simplicial vertices of $G$. By Observation~\ref{obs:simplicial}, any geodetic set of $G$ contains all simplicial vertices of $G$. %Thus, if $k-|S|<0$, we return \no.
Now, notice that $X\cup S$ is a geodetic set of $G$. Indeed, any vertex $v$ from $I$ that is not simplicial has two non-adjacent neighbors $x,y$ in $X$, and thus, $v$ is covered by $x$ and $y$ (which are at distance~2 from each other).

Hence, to enumerate all possible minimum-size geodetic sets, it suffices to enumerate all subsets $S'$ of vertices of size at most $|X|$ in $(X \cup I) \setminus S$, and check whether $S\cup S'$ is a geodetic set. If one such set is indeed a geodetic set and has size at most $k$, we return \yes. Otherwise, we return \no. The statement follows.
\end{proof}


==> algo-vertex-cover-MD.tex <==
%\section{\mdfull: Algorithms for Vertex Cover Parameterization}
\subsection{Algorithm for \mdfull}
\label{sec:algo-fpt-vertex-cover}

To prove Theorem~\ref{thm:algo-vertex-cover} for \mdfull, we first show the following.

\begin{lemma}
\label{lemma:kernel-vc}
\textsc{Metric Dimension},  parameterized by the vertex cover number $\vc$,
admits a polynomial-time kernelization algorithm that returns an instance
with 
$2^{\OO(\vc)}$ vertices.
\end{lemma}
\begin{proof}
Given a graph $G$,  let $X\subseteq V(G)$ be a minimum vertex cover of $G$. 
If such a vertex cover is not given, then we can find a $2$-factor approximate vertex
cover in polynomial time. 
Let $I:=V(G)\setminus X$.
By the definition of a vertex cover, the vertices of $I$ are pairwise non-adjacent.
%That is, $I$ induces an independent set in $G$.
The kernelization algorithm exhaustively applies the following reduction rule.
\begin{reduction rule} 
\label{reduc:twins}
If there exist three vertices $u,v,  x\in I$ such that $u,v, x$ are false twins, 
then delete $x$ and decrease $k$ by one.
\end{reduction rule}
Since $u,v, x$ are false twins, $N(u)=N(v)=N(x)$. 
This implies that, for any vertex $w\in V(G)\setminus \{u,v, x\}$, $d(w,v)=d(w,u)=d(w, x)$. 
Hence, any resolving set that excludes at least two vertices in $\{u, v, x\}$
cannot resolve all three pairs $\{u,v\}$,  $\{u, x\}$,  and $\{v, x\}$.
As the vertices in $\{u, v, x\}$ are distance-wise indistinguishable
from the remaining vertices, we can assume, without loss of generality, that 
any resolving set contains both $u$ and $x$.
Hence, any pair of vertices in $V(G) \setminus \{u, x\}$ that 
is resolved by $x$ is also resolved by $u$.
In other words, if $S$ is a resolving set of $G$, then
$S \setminus \{x\}$ is a resolving set of $G - \{x\}$.
This implies the correctness of the forward direction.
The correctness of the reverse direction trivially follows from the fact
that we can add $x$ into a resolving set of $G - \{x\}$
to obtain a resolving set of $G$.

Consider an instance on which the reduction rule is not applicable.
If the budget is negative, then the algorithm returns a trivial \no-instance
of constant size.
Otherwise, for any $Y\subseteq X$, there are at most two vertices $u,v\in I$ such that $N(u)=N(v)=Y$.
This implies that the number of vertices in the reduced instance
is at most $|X| + 2 \cdot 2^{|X|} =  2^{\vc +1} + \vc$.
\end{proof}

Next, we present an \XP-algorithm parameterized by the vertex 
cover number. 
This algorithm, along with the kernelization algorithm above,
imply that \textsc{Metric Dimension} admits
an algorithm running in time $2^{\calO(\vc^2)}\cdot n^{\calO(1)}$.

\begin{lemma}
\label{lemma:algo-xp-vc}
\textsc{Metric Dimension} admits an algorithm running in time $n^{\calO(\vc)}$.
\end{lemma}
\begin{proof}
The algorithm starts by computing a minimum vertex cover $X$ of $G$ 
in time $2^{\mathcal{O}(\vc)} \cdot n^{\calO(1)}$ using an \FPT\ algorithm
for the \textsc{Vertex Cover} problem, for example the one in~\cite{DBLP:journals/jal/ChenKJ01}.
Let $I := V(G)\setminus X$. 
Then,  in polynomial time, it computes a largest subset $F$ of $I$ such that, 
for every vertex $u$ in $F$,  $I \setminus F$ contains a false twin of $u$.
By the arguments in the previous proof,  if there are false twins in $I$,  say $u, v$,
then any resolving set contains at least one of them.
Hence,  it is safe to assume that any resolving set contains $F$.
%If $k' \ge |X|$,  then the algorithm returns \yes.
If $k - |F| < 0$, then the algorithm returns \no.
Otherwise,  it enumerates every subset of vertices of size at most $|X|$ in $X \cup (I \setminus F)$. 
If there exists a subset $A \subseteq X \cup (I \setminus F)$ 
such that $A\cup F$ is a resolving set of $G$ of size at most $k$,
then it returns $A\cup F$.
Otherwise,  it returns \no.

In order to prove that the algorithm is correct, we prove that $X \cup F$ is a resolving set of $G$.
It is easy to see that, for a pair of distinct vertices $u,v$,
if $u \in X \cup F$ and $v \in V(G)$,  then the pair is resolved by $u$.
It remains to argue that every pair of distinct vertices in $(I \setminus F) \times (I \setminus F)$ is
resolved by $X \cup F$.
Note that, for any two vertices $u, v\in I \setminus F$,  $N(u) \neq N(v)$ as otherwise 
$u$ can be moved to $F$, contradicting the maximality of $F$.
Hence, there is a vertex in $X$ that is adjacent to $u$, but not adjacent to $v$,
resolving the pair $\langle u, v\rangle$.
This implies the correctness of the algorithm.
The running time of the algorithm easily follows from its description. 
\end{proof}

==> lower-bound-vertex-cover-MD.tex <==
\section{\mdfull: Lower Bounds Regarding Vertex Cover}
\label{sec:lower-bound-vertex-cover}

In this section, we first prove
the following theorem.

\begin{theorem}
\label{thm:reduction-3-SAT-Met-Dim-VC}
There is an algorithm that, given an instance
$\psi$ of \textsc{3-Partitioned-3-SAT} on $N$ variables,  
runs in time $2^{\calO(\sqrt{N})}$, and constructs an equivalent 
instance $(G, k)$ of \mdfull such that 
$\vc(G) + k = \OO(\sqrt{N})$ (and $|V(G)| = 2^{\OO(\sqrt{N})}$).
\end{theorem}

The above theorem, along with the 
arguments that are standard to prove 
the \ETH-based lower bounds, 
immediately implies the following 
results.


\begin{corollary}
\label{cor:MD-vc-lower-bound-algo}
Unless the \ETH\ fails, 
\mdfull does not admit an algorithm 
running in time $2^{o(\vc^2)} \cdot n^{\OO(1)}$. 
\end{corollary}
\begin{corollary}
\label{cor:MD-vc-lower-bound-kernel}
Unless the \ETH\ fails, 
\mdfull does not admit a kernelization algorithm that
reduces the solution size $k$ and
outputs a kernel with $2^{o(k + \vc)}$ vertices. 
\end{corollary}
\begin{proof}[Proof assuming 
Theorem~\ref{thm:reduction-3-SAT-Met-Dim-VC}]
For the sake of contradiction, assume that such a kernelization algorithm exists.
Consider the following algorithm for \textsc{$3$-SAT}.
Given a \textsc{$3$-SAT} formula on $N$ variables, 
it uses Theorem~\ref{thm:reduction-3-SAT-Met-Dim-VC} to obtain
an equivalent instance of $(G, k)$ such that $\vc(G) + k = \calO(\sqrt{N})$ and $|V(G)| = 2^{\OO(\sqrt{N})}$.
Then,  it uses the assumed kernelization algorithm
to construct an equivalent instance $(H, k')$ such that 
$H$ has $2^{o(\vc(G) + k)}$ vertices and
$k' \le k$.
Finally,  it uses a brute-force algorithm,  running in time $|V(H)|^{\calO(k')}$,
to determine whether the reduced instance, or equivalently the input
instance of \textsc{$3$-SAT},  is a \yes-instance.
The correctness of the algorithm follows from the 
correctness of the respective algorithms and our assumption.
The total running time of the algorithm is 
$2^{\calO(\sqrt{N})} + (|V(G)| + k)^{\calO(1)} + |V(H)|^{\calO(k')}
= 2^{\calO(\sqrt{N})} + (2^{\calO(\sqrt{N})})^{\calO(1)} + (2^{o(\sqrt{N})})^{\calO(\sqrt{N})}
= 2^{o(N)}$.
But this contradicts the \ETH.
\end{proof}


For the reduction, we will be using some of the tools introduced in \Cref{subsec:prelim-3-Par-3-SAT-Met-Dim-diam-tw}.

%\subsection{Preliminary Tools}
%\label{subsec:prelim-3-Par-3-SAT-Met-Dim}
%\begin{figure}[t]
%    \centering
%        \includegraphics[scale=0.93]{./images/set-identifying-gadget2.pdf} \hspace{0.4cm}
%        \includegraphics[scale=0.93]{./images/vertex-selector-gadget2.pdf}
%    \caption{ \textbf{Set Identifying Gadget (left)}. The blue box represents $\bitrep(X)$ and the yellow lines represent that every vertex in $\bitrep(X)$ is adjacent to $\bitrepnullifier(X)$, $\bitrepnullifier(X)$ is adjacent to every vertex in $N(X)$, and $y_{\star}$ is adjacent to every vertex in $X$. Note that $G'$ is not necessarily restricted to the graph induced by the vertices in $X\cup N(X)$.
%    \textbf{Vertex Selector Gadget (right)}.
%    For $X \in \{B,  A\}$,  the blue box represents $\bitrep(X)$, the blue link represents the connection
%    with respect to the binary representation, and the yellow line represents that $\bitrepnullifier(X)$
%    is connected to every vertex in the set.
%    The dotted lines highlight the absence of edges.}
%    \label{fig:set-identifying-gadget}
%    \label{fig:vertex-selector-gadget}
%\end{figure}
%
%\subsubsection{Set Identifying Gadget}
%\label{subsubsec:gadget-set}
%
%Suppose we are given a graph $G'$ and a subset $X\subseteq V(G')$ of its vertices.
%Further, suppose that we want to add a vertex set $X^+$ to $G'$ in order to obtain a new graph $G$ with the following properties. We want that each vertex in $X \cup X^+$ will be distinguished by vertices in $X^+$ that must be in any resolving set $S$ of $G$, and no vertex in $X^+$ can resolve any ``critical pair'' of vertices in $V(G)$ (critical pairs will be defined in the next subsection).
% 
%We refer to the graph induced by the vertices of $X^+$, along with the edges connecting $X^+$ to $G'$, as the Set Identifying Gadget for the set $X$.
%
%Given a graph $G'$ and a non-empty subset $X\subseteq V(G')$ of its vertices, to construct such a graph $G$, we add vertices and edges to $G'$ as follows:
%\begin{itemize}
%\item The vertex set $X^+$ that we are aiming to add is the union of a set $\bitrep(X)$ and a special vertex denoted by $\bitrepnullifier(X)$.
%\item First, let $X=\{x_i\mid i\in [|X|]\}$, and set $q := \lceil \log(|X|+ 2) \rceil+1$.
%We select this value for $q$ to \emph{(1)} uniquely represent each integer in $[|X|]$ by its bit-representation in binary (note that we start from $1$ and not $0$), \emph{(2)} ensure that the only vertex whose bit-representation contains all $1$'s is $\bitrepnullifier(X)$, and \emph{(3)} reserve one spot for an additional vertex $y_{\star}$.
%\item For every $i \in [q]$, add three vertices $y^a_i,  y_i, y^b_i$, and add the path $(y^a_i, y_i, y^b_i)$.
%\item Add three vertices $y^a_{\star},  y_{\star}, y^b_{\star}$, and add the path $(y^a_{\star}, y_{\star}, y^b_{\star})$. 
%Add all the edges to make $\{y_i\mid\ i \in [q] \}\cup\{y_{\star}\}$ into a clique.
%Make $y_{\star}$ adjacent to each vertex $v\in X$.
%We denote $\bitrep(X)=\{y_i, y^a_i, y^b_i\mid i\in [q]\}\cup \{y_{\star}, y^a_{\star}, y^b_{\star}\}$ and its subset $\bits(X)=\{y^a_i, y^b_i\mid i\in [q]\}\cup \{y^a_{\star}, y^b_{\star}\}$ for convenience in a later case analysis.
%\item For every integer $j \in [|X|]$, let $\bit(j)$ denote the binary
%representation of $j$ using $q$ bits.
%Connect $x_j$ with $y_{i}$
%if the $i^{th}$ bit (going from left to right) in $\bit(j)$ is $1$.
%\item Add a vertex, denoted by $\bitrepnullifier(X)$,
%and make it adjacent to every vertex in $\{y_i\mid i \in [q] \}\cup\{y_{\star}\}$.
%One can think of the vertex $\bitrepnullifier(X)$ as the only vertex whose bit-representation contains all $1$'s.
%\item For every vertex $u \in V(G)\setminus (X\cup X^+)$ such that
%$u$ is adjacent to some vertex in $X$, add an edge between
%$u$ and $\bitrepnullifier(X)$.
%We add this vertex to ensure that
%vertices in $\bitrep(X)$ do not resolve critical pairs
%in $V(G)$.
%\end{itemize}
%This completes the construction of $G$. The properties of $G$ are not proven yet, but just given as an intuition behind its construction. See Figure~\ref{fig:set-identifying-gadget} for an illustration.
%
%\subsubsection{Gadget to Add Critical Pairs}
%\label{subsubsec:gadget-critical-pairs}
%Any resolving set needs to resolve \emph{all} pairs of vertices in
%the input graph.
%As we will see, some pairs, which we call critical pairs are harder
%to resolve than others.
%In fact, the non-trivial part will be to
%resolve all of the critical pairs.
%
%Suppose we need to have many critical pairs in a graph $G$, say $\langle c^\circ_i,   c^\star_i \rangle$
%for every $i \in [m]$ for some $m \in \mathbb{N}$.
%Define $C := \{c^{\circ}_i,  c^{\star}_i\mid i \in [m]\}$.
%We then add $\bitrep(C)$ and $\bitrepnullifier(C)$ as mentioned above (taking $C$ as the set $X$), but
%the connection across $\{c^{\circ}_i, c^\star_i\}$ and $\bitrep(C)$ is defined by $\bit(i)$, i.e.,
%connect both $c^{\circ}_i$ and $c^\star_i$ with the $j$-th vertex of $\bitrep(C)$
%if the $j^{th}$ digit (going from left to right) in $\bit(i)$ is $1$.
%Hence,  $\bitrep(C)$ can resolve any pair of the form
%$\langle c^{\circ}_i,  c^{\star}_{\ell} \rangle$,  $\langle c^{\circ}_i,  c^{\circ}_{\ell} \rangle$,  or
%$\langle c^{\star}_i,  c^{\star}_{\ell} \rangle$ as long as $i \neq \ell$.
%As before, $\bitrep(C)$ can also resolve all pairs with one vertex in
%$C \cup \bitrep(C) \cup \{\bitrepnullifier(C)\}$, but no critical pair of vertices. Again, when these facts
%will be used, they will be proven formally.
%
%\subsubsection{Vertex Selector Gadgets}
%\label{subsubsec:vertex-selector}
%
%
%Suppose we are given a collection of sets $A_1, A_2, \dots, A_q$ of vertices
%in a graph $G$, and
%we want to ensure that any resolving set of $G$ includes at least one vertex
%from $A_i$ for every $i \in [q]$.
%In the following,  we construct a gadget that achieves a slightly weaker objective.
%\begin{itemize}
%\item Let $A = \underset{i \in [q]}{\bigcup} A_i$.
%Add a set identifying gadget for $A$ as mentioned in Subsection~\ref{subsubsec:gadget-set}.
%\item For every $i \in [q]$,  add two vertices $b^{\circ}_i$ and $b^{\star}_i$.
%Use the gadget mentioned in Subsection~\ref{subsubsec:gadget-critical-pairs}
%to make all the pairs of the form
%$\langle b^{\circ}_i, b^{\star}_i \rangle$ critical pairs.
%
%\item For every $a \in A_i$,  add an edge $(a, b^{\circ}_i)$.
%We highlight that we do not make $a$ adjacent to $b^{\star}_i$
%by a dotted line in Figure~\ref{fig:vertex-selector-gadget}.
%Also, add the edges $(a,  \bitrepnullifier(B))$,  $(b^{\circ}_i,  \bitrepnullifier(A))$, $(b^{\star}_i,  \bitrepnullifier(A))$, and $(\bitrepnullifier(A), \bitrepnullifier(B))$.
%\end{itemize}
%This completes the construction.
%
%Note that the only vertices that can resolve a critical pair $\langle b^{\circ}_i, b^{\star}_i \rangle$,
%apart from $b^{\circ}_i$ and $b^{\star}_i$, are the vertices in $A_i$.
%Hence, every resolving set contains at least one vertex in
%$\{b^{\circ}_i, b^{\star}_i\} \cup A_i$. Again, when used, these facts will be proven formally.
%
\subsection{Reduction}
\label{subsec:reduction-3-Par-3-SAT-Met-Dim}

%In this subsection,  we present a reduction from
%\textsc{3-Partitioned-3-SAT} to \textsc{Metric Dimension}.
%As mentioned before, this version of \textsc{3-SAT} was introduced
%in~\cite{DBLP:journals/corr/abs-2302-09604} and is defined as follows.
%
%\defproblem{\textsc{3-Partitioned-3-SAT}}{A formula $\psi$ in $3$-\textsc{CNF} form,
%together with a partition of the set of its variables into three
%disjoint sets $X^{\alpha}$, $X^{\beta}$, $X^{\gamma}$,
%with $|X^{\alpha}| = |X^{\beta}| = |X^{\gamma}| = n$, and
%such that no clause contains more than one variable from each of
%$X^{\alpha},  X^{\beta}$, and $X^{\gamma}$.}{Determine whether $\psi$ is satisfiable.}
%
%The authors of~\cite{DBLP:journals/corr/abs-2302-09604} also proved the following.
%
%\begin{proposition}[{\cite[Theorem 3]{DBLP:journals/corr/abs-2302-09604}}]
%\label{prop:3-SAT-to-3-Partition-3-SAT}
%Unless the \ETH\ fails,  \textsc{3-Partitioned-3-SAT} does not admit
%an algorithm running in time $2^{o(n)}$.
%\end{proposition}

Consider an instance $\psi$ of \textsc{3-Partitioned-3-SAT}
with $X^{\alpha}, X^{\beta}, X^{\gamma}$ the partition of the variable set.
By adding dummy variables in each of these sets, we can assume that $\sqrt{n}$ is an integer.
From $\psi$, we construct the graph $G$ as follows.
We describe the construction of $X^{\alpha}$, with the constructions for $X^{\beta}$ and $X^{\gamma}$ being analogous.
We rename the variables in $X^{\alpha}$
to $x^{\alpha}_{i, j}$ for $i, j \in [\sqrt{n}]$.

\begin{itemize}
\item We partition the variables of $X^{\alpha}$ into \emph{buckets}
$X^{\alpha}_1,  X^{\alpha}_2,  \dots ,X^{\alpha}_{\sqrt{n}}$
such that each bucket contains $\sqrt{n}$ many variables.
Let $X^{\alpha}_i = \{x^{\alpha}_{i, j}\ |\ j \in [\sqrt{n}]\}$ for all $i\in [\sqrt{n}]$.

\item For every $X^{\alpha}_i$, we construct the set $A^{\alpha}_i$ of $2^{\sqrt{n}}$ new vertices, $A^{\alpha}_i=\{a^{\alpha}_{i,  \ell}\mid \ell \in [2^{\sqrt{n}}]\}$.
Each vertex in $A^{\alpha}_i$ corresponds to a certain possible assignment of
variables in $X^{\alpha}_i$.
Let $A^{\alpha}$ be the collection of all the vertices added in the above step.
Formally,   $A^{\alpha} = \{a^{\alpha}_{i, \ell} \in A_i |\ i \in [\sqrt{n}] \text{ and }
\ell \in [2^{\sqrt{n}}]  \}$.
We add a set identifying gadget as mentioned in
Subsection~\ref{subsubsec:gadget-set-MD} in order to resolve every pair of vertices in $A^{\alpha}$.

\item For every $X^{\alpha}_i$, we construct a pair
$\langle b^{\alpha, \circ}_i, b^{\alpha, \star}_i \rangle$ of vertices.
Then, we add a gadget to make the pairs
$\{\langle b^{\alpha, \circ}_i, b^{\alpha, \star}_i \rangle\mid i\in [\sqrt{n}]\}$ critical as mentioned in Subsection~\ref{subsubsec:gadget-critical-pairs}.
Let $B^{\alpha} = \{b^{\alpha, \circ}_i, b^{\alpha, \star}_i\  |\ i \in [\sqrt{n}] \}$
be the collection of vertices in the critical pairs.
We add edges in $B^{\alpha}$ to make it a clique.

\item We would like that
any resolving set contains at least one vertex in $A^{\alpha}_i$
for every $i \in [\sqrt{n}]$, but instead we add the construction from Subsection~\ref{subsubsec:vertex-selector} that achieves the slightly weaker objective as mentioned there.
However,  for every $A^{\alpha}_i$,  instead of adding two new vertices, we use
$\langle b^{\alpha, \circ}_i,  b^{\alpha,  \star}_i \rangle$ as the necessary critical pair.
Formally,  for every $i \in [\sqrt{n}]$,  we make $b^{\alpha, \circ}_i$ adjacent to every vertex
in $A^{\alpha}_{i}$.
We add edges to make $\bitrepnullifier(B^{\alpha})$ adjacent to every vertex
in $A^{\alpha}$, and
$\bitrepnullifier(A^{\alpha})$ adjacent to every vertex in $B^{\alpha}$.
Recall that there is also the edge $(\bitrepnullifier(B^{\alpha}), \bitrepnullifier(A^{\alpha}))$.


\item We add \emph{portals} that transmit information
from vertices corresponding to assignments, i.e., vertices in $A^{\alpha}$,
to critical pairs corresponding to clauses, i.e., vertices in $C$
{which we define soon}.
A portal is a clique on $\sqrt{n}$ vertices in the graph $G$.
We add three portals, the \emph{truth portal} (denoted by $T^{\alpha}$),
\emph{false portal} (denoted by $F^{\alpha}$), and
\emph{validation portal} (denoted by $V^{\alpha}$).
Let
$T^{\alpha} = \{t^{\alpha}_1,  t^{\alpha}_2, \dots, t^{\alpha}_{\sqrt{n}}\}$,
$F^{\alpha} = \{f^{\alpha}_1,  f^{\alpha}_2, \dots, f^{\alpha}_{\sqrt{n}}\}$,
and
$V^{\alpha} = \{v^{\alpha}_1,  v^{\alpha}_2, \dots, v^{\alpha}_{\sqrt{n}}\}$.
Moreover,  let $P^{\alpha} = V^{\alpha} \cup T^{\alpha} \cup F^{\alpha}$.

\item We add a set identifying gadget to $P^{\alpha}$ as mentioned
in Subsection~\ref{subsubsec:gadget-set-MD}.
We add an edge between $\bitrepnullifier(A^{\alpha})$ and every vertex of $P^{\alpha}$; and the edge $(\bitrepnullifier(P^{\alpha}),  \bitrepnullifier(A^{\alpha}))$.
However, we note that we \emph{do not} add edges across
$\bitrepnullifier(P^{\alpha})$ and $A^{\alpha}$, as can be seen in Figure~\ref{fig:reduction-overview}.
Lastly, we add edges in $P^{\alpha}$ to make it a clique.

\item We add edges across $A^{\alpha}$ and the portals as follows.
For $i \in [\sqrt{n}]$ and $\ell \in [2^{\sqrt{n}}]$,
consider a vertex $a^{\alpha}_{i, \ell}$ in $A^{\alpha}_i$.
Recall that this vertex corresponds to an assignment
$\pi: B^{\alpha}_i \mapsto \{\true, \false\}$,
where $B_i^{\alpha}$ is the collection of variables
$\{x^{\alpha}_{i, j}\ |\ j \in [\sqrt{n}] \}$.
If $\pi(x^{\alpha}_{i, j}) = \true$, then we add the edge $(a^{\alpha}_{i,  \ell},  t^{\alpha}_j)$.
Otherwise,  $\pi(x^{\alpha}_{i, j}) = \false$, and we add the edge
$(a^{\alpha}_{i,  \ell},  f^{\alpha}_j)$.
We add the edge $(a^{\alpha}_{i,  \ell},  v^{\alpha}_{i})$ for every $\ell \in [2^{\sqrt{n}}]$.
\end{itemize}

Then, we repeat the above steps to construct
$B^{\beta},  A^{\beta},  P^{\beta}$,
$B^{\gamma},  A^{\gamma},  P^{\gamma}$.

\begin{figure}[H]
    \centering
        \includegraphics[scale=1]{./images/reduction-overview2.pdf}
    \caption{Overview of the reduction.
    Sets with elliptical boundaries are independent sets, and sets with rectangular boundaries are cliques.
    For the set $X \in \{B^{\alpha}, A^{\alpha},  P^{\alpha}, C\}$,  the blue rectangle attached to it
    via the blue edge represents $\bitrep(X)$.
    {We do not show $\bits(X)$ for the sake of clarity.}
    The yellow thick line represents that $\bitrepnullifier(X)$ is connected to every vertex in the set.
    Note the exception of $\bitrepnullifier(P^{\alpha})$ which is \emph{not} adjacent to any
    vertex in $A^{\alpha}$.
    Purple lines across two sets denote adjacencies with respect to indexing,
    i.e.,  $b^{\alpha, \circ}_i$ is adjacent only with all the vertices in $A^{\alpha}_{i}$,
    and all the vertices in $A^{\alpha}_i$ are adjacent with $v^{\alpha}_i$ in
    validation portal $V^{\alpha}$.
    Gray lines also indicate adjacencies with respect to indexing, but in a complementary
    way.
    If $C_q$ contains a variable in $B^{\alpha}_i$, then $c^{\circ}_q$ and $c^{\star}_q$
    are adjacent with all vertices $v^{\alpha}_j \in V^{\alpha}$ such that $j \neq i$.
    The green and red lines across the $A^{\alpha}$ and $T^{\alpha}$ and $F^{\alpha}$ transfer, in some sense, for each $a_{i,\ell}^{\alpha}\in A^{\alpha}$, the underlying assignment structure.
    If the $j^{th}$ variable by $a_{i,\ell}^{\alpha}$ is assigned to \true, then we add the green edge $(a_{i,\ell}^{\alpha}, t_{j}^{\alpha})$, and otherwise the red edge $(a_{i,\ell}^{\alpha}, f_{j}^{\alpha})$.
    Similarly, we add edges for each $c_i^{\circ}\in C$ depending on the assignment (\true\ or \false) satisfying the variable from the part $X^{\delta}$ of a clause $c_i$, and in which block $B_j^{\delta}$ it lies, putting either an edge $(c_i^{\circ},t_j^{\delta})$ or $(c_i^{\circ},f_j^{\delta})$ accordingly.
    {Here,  $\delta \in \{\alpha, \beta, \gamma\}$.}
    }
    \label{fig:reduction-overview}
\end{figure}

Now, we are ready to proceed through the final steps to complete the construction.
\begin{itemize}
\item For every clause $C_q$ in $\psi$,  we introduce a pair of vertices
$\langle c^{\circ}_q,  c^{\star}_q \rangle$.
Let $C$ be the collection of vertices in such pairs.
Then, we add a gadget as was described in Subsection~\ref{subsubsec:gadget-critical-pairs} to make each pair
$\langle c^{\circ}_q,  c^{\star}_q \rangle$ a critical one.


\item We add edges across $C$ and the portals as follows for each $\delta \in \{\alpha, \beta, \gamma\}$.
Consider a clause $C_q$ in $\psi$ and the corresponding
critical pair $\langle c^{\circ}_q,  c^{\star}_q \rangle$ in $C$.
As $\psi$ is an instance of \textsc{$3$-Partitioned-$3$-SAT},
there is at most one variable in $X^{\delta}$ that appears in $C_q$.
Suppose that variable is $x^{\delta}_{i, j}$ for some $i, j \in [\sqrt{n}]$.
The first subscript decides the edges across
$\langle c^{\circ}_q,  c^{\star}_q \rangle$ and the validation portal,
whereas the second subscript decides the edges across
$\langle c^{\circ}_q,  c^{\star}_q \rangle$ and
either the truth portal or false portal in the following sense.
If $x^{\delta}_{i, j}$ appears in $C_q$, then we add all edges of the form
$(v^{\delta}_{i'},  c^{\circ}_q)$ and $(v^{\delta}_{i'},  c^{\star}_q)$
for every $i' \in [\sqrt{n}]$ such that $i' \neq i$.
If $x^{\delta}_{i, j}$ appears as a positive literal in $C_q$, then we add the edge $(t^{\delta}_j,  c^{\circ}_q)$.
If $x^{\delta}_{i, j}$ appears as a negative literal in $C_q$, then we add the edge $(f^{\delta}_j,  c^{\circ}_q)$.
Note that if $C_q$ does not contain a variable in $X^{\delta}$,
then we make $c^{\circ}_q$ and $c^{\star}_q$
adjacent to every vertex in $V^{\delta}$, whereas they
are not adjacent to any vertex in $T^{\delta} \cup F^{\delta}$.
Finally, we add an edge between $\bitrepnullifier(P^{\delta})$ and every vertex of $C$, and we add the edge $(\bitrepnullifier(P^{\delta}),  \bitrepnullifier(C))$.
\end{itemize}

This concludes the construction of $G$.
The reduction returns $(G,  k)$
as an instance of \textsc{Metric Dimension} where
\begin{equation*}
\begin{split}
k &= 3 \cdot \left(\sqrt{n} + \left(\left\lceil\log(|B^{\alpha}|/2 + 2)\right\rceil + 1\right)
+ \left(\left\lceil\log(|A^{\alpha}|+ 2)\right\rceil + 1\right) + \left(\left\lceil\log(|P^{\alpha}|+ 2)\right\rceil + 1\right) \right) +
\\
&  \lceil\log(|C|+ 2)\rceil + 1.
\end{split}
\end{equation*}

%\subsection{Correctness of the Reduction}\label{subsec:correctness-3-Par-3-SAT-Met-Dim}

\begin{figure}[H]
    \centering
        \includegraphics[scale=1.25]{./images/reduction-core2.pdf}
    \caption{A toy example to illustrate the core ideas in the reduction. Note that $\bitrep$ and $\bitrepnullifier$ are omitted for the sets.}
    \label{fig:reduction-core}
\end{figure}

We give an informal description of the proof of correctness here.
See Figure~\ref{fig:reduction-core}.
Suppose $\sqrt{n} = 3$ and the vertices in the sets are indexed from top to bottom.
For the sake of clarity,  we do not show all the edges and only show $4$ out of $8$ vertices
in each $A^{\alpha}_i$ for $i \in [3]$.
We also omit $\bitrep$ and $\bitrepnullifier$ for these sets.
The vertex selection gadget and the budget $k$ ensure that exactly one vertex in
$\{b^{\alpha,\circ}_i,  b^{\alpha,\star}_i\} \cup A^{\alpha}_i$ is selected for every $i \in [3]$.
If a resolving set contains a vertex from $A^{\alpha}_i$,
then it corresponds to selecting an assignment of variables in $X^{\alpha}_i$.
For example,  the vertex $a^{\alpha}_{2, 2}$ corresponds to the assignment
$\pi: X^{\alpha}_2 \mapsto \{\true, \false\}$.
Suppose $X^{\alpha}_2 = \{x^{\alpha}_{2, 1},  x^{\alpha}_{2, 2},  x^{\alpha}_{2, 3}\}$,
$\pi(x^{\alpha}_{2, 1}) = \pi(x^{\alpha}_{2,3}) = \true$, and $\pi(x^{\alpha}_{2, 2}) = \false$.
Hence,  $a^{\alpha}_{2, 2}$ is adjacent to the first and third vertex in the truth portal $T^{\alpha}$,
whereas it is adjacent with the second vertex in the false portal $F^{\alpha}$.
Suppose the clause $C_q$ contains the variable $x^{\alpha}_{2, 1}$ as a positive literal.
Note that $c^{\circ}_q$ and $c^{\star}_q$ are at distance $2$ and $3$,  respectively,  from
$a^{\alpha}_{2, 2}$.
Hence, the vertex $a^{\alpha}_{2, 2}$, corresponding to the assignment $\pi$ that satisfies clause $C_q$,
resolves the critical pair $\langle c^{\circ}_q,  c^{\star}_q \rangle$.
Now, suppose there is another assignment $\sigma: X^{\alpha}_3 \mapsto \{\true, \false\}$ such that
$\sigma(x^{\alpha}_{3, 1}) = \sigma(x^{\alpha}_{3,3}) = \true$ and $\sigma(x^{\alpha}_{3, 2}) = \false$.
As $\psi$ is an instance of \textsc{$3$-Partitioned-$3$-SAT}
and $C_q$ contains a variable in $X^{\alpha}_2$ ($ \subseteq X^{\alpha}$),
$C_q$ does not contain a variable in $X^{\alpha}_3$ ($\subseteq X^{\alpha}$).
Hence,  $\sigma$ does not satisfy $C_q$.
Let $a^{\alpha}_{3, 2}$ be the vertex in $X^{\alpha}_3$ corresponding to $\sigma$.
The connections via the validation portal $V^{\alpha}$ ensure that
both $c^{\circ}_q$ and $c^{\star}_q$ are at distance $2$ from
$a^{\alpha}_{3, 2}$, and hence, $a^{\alpha}_{3, 2}$ cannot resolve the
critical pair $\langle c^{\circ}_q,  c^{\star}_q \rangle$.
Hence,  finding a resolving set in $G$ corresponds to finding a satisfying
assignment for $\psi$. These intuitions are formalized in the following subsection.

\subsection{Correctness of the Reduction}

Suppose, given an instance $\psi$ of \textsc{$3$-Partitioned-$3$-SAT}, that the reduction of this subsection returns $(G, k)$ as an instance of \textsc{Metric Dimension}. We first prove the following lemma which will be helpful in proving the correctness of the reduction.

\begin{lemma} For any resolving set $S$ of $G$ and for all $X\in \{B^{\delta},A^{\delta},P^{\delta},C\}$ and $\delta\in \{\alpha,\beta,\gamma\}$,
\begin{enumerate}
\item $S$ contains at least one vertex from each pair of false twins in $\bits(X)$.
\item Vertices in $\bits(X) \cap S$ resolve any non-critical pair of vertices
$\langle u, v\rangle$ when $u \in X\cup X^+$ and $v\in V(G)$.  
\item Vertices in $X^+ \cap S$ \emph{cannot} resolve any critical
pair of vertices $\langle b_i^{\delta',\circ},  b_i^{\delta',\star}\rangle$ nor $\langle c_q^{\circ},  c_q^{\star}\rangle$ for all $i\in [\sqrt{n}]$, $\delta'\in \{\alpha,\beta,\gamma\}$, and $q\in [m]$.     
\end{enumerate}\label{claim:set-ind}
\end{lemma}
\begin{proof}
\begin{enumerate}
\item By~\cref{obs:twins}, the statement follows for all $X\in \{B^{\delta},A^{\delta},P^{\delta},C\}$ and $\delta\in \{\alpha,\beta,\gamma\}$.

\item For all $X\in \{B^{\delta},A^{\delta},P^{\delta},C\}$ and $\delta\in \{\alpha,\beta,\gamma\}$, note that $\bitrepnullifier(X)$ is distinguished by $\bits(X)$ since it is the only vertex in $G$ that is at distance~$2$ from every vertex in $\bits(X)$. We now do a case analysis for the remaining non-critical pairs of vertices $\langle u, v \rangle$ assuming that $\bitrepnullifier(X)\notin \{u,v\}$ (also, suppose that both $u$ and $v$ are not in $S$, as otherwise, they are obviously distinguished):
\begin{description}
\item[Case i: $u, v \in X\cup X^+$.]
\hfill
\begin{description}
\item[Case i(a): $u, v\in X$ or $u, v\in \bitrep(X)\setminus \bits(X)$.] In the first case, let $j$ be the digit in the binary representation of the subscript of $u$ that is not equal to the $j^{\text{th}}$ digit in the binary representation of the subscript of $v$ (such a $j$ exists since $\langle u, v \rangle$ is not a critical pair). In the second case, without loss of generality, let $u=y_i$ and $v=y_j$. 
By the first item of the statement of the lemma (1.), without loss of generality, $y_j^{a}\in S\cap \bits(X)$.
Then, in both cases, $d(y_j^a, u)\neq d(y_j^a, v)$.
\item[Case i(b): $u \in X$ and $v\in \bitrep(X)$.]
Without loss of generality, $y_{\star}^{a}\in S\cap \bits(X)$ (by 1.). 
Then, $d(y_{\star}^{a}, u)=2$ and, for all $v\in \bits(X)\setminus\{y_{\star}^b\}$, $d(y_{\star}^{a}, v)=3$. 
Without loss of generality, let $y_i$ be adjacent to $u$ and let $y_i^a\in S\cap \bits(X)$ (by 1.).
Then, for $v=y_{\star}^b$, $3=d(y_i^a, v)\neq d(y_i^a, u)=2$.
If $v\in \bitrep(X)\setminus \bits(X)$, then, without loss of generality, $v=y_j$ and $y_j^a\in S\cap \bits(X)$ (by 1.), and $1=d(y_j^a, v)< d(y_j^a, u)$.
\item[Case i(c): $u, v\in \bits(X)$.]
Without loss of generality, $u=y_i^b$ and $y_i^a\in S$ (by 1.). 
Then, $2=d(y_i^a, u)\neq d(y_i^a, v)=3$.
\item[Case i(d): $u \in \bits(X)$ and $v\in \bitrep(X)\setminus \bits(X)$.]
Without loss of generality, $v=y_i$ and $y_i^a\in S$ (by 1.). 
Then, $1=d(y_i^a, v) < d(y_i^a, u)$.
\end{description}
\item[Case ii: $u \in X\cup X^+$ and $v \in V(G)\setminus (X\cup X^+)$.]
For each $u \in X\cup X^+$, there exists $w\in \bits(X)\cap S$ such that $d(u, w)\leq 2$, while, for each $v \in V(G)\setminus (X\cup X^+)$ and $w\in \bits(X)\cap S$, we have $d(v, w)\geq 3$.
\end{description}
\item For all $X\in \{B^{\delta},A^{\delta},P^{\delta}\}$, $\delta\in \{\alpha,\beta,\gamma\}$, $u\in X^+$, $v \in \{c_q^{\circ}, c_q^{\star}\}$, and $q\in [m]$,
we have that $d(u, v)=d(u, \bitrepnullifier(P^{\delta}))+1$.
Further, for $X=C$ and all $u\in X^+$ and $q\in [m]$, either $d(u,c_q^{\circ})=d(u,c_q^{\star})=1$, $d(u,c_q^{\circ})=d(u,c_q^{\star})=2$, or $d(u,c_q^{\circ})=d(u,c_q^{\star})=3$ by the construction in Subsection~\ref{subsubsec:gadget-critical-pairs} and since $\bitrep(X)\setminus \bits(X)$ is a clique. 
Hence, for all $X\in \{B^{\delta},A^{\delta},P^{\delta},C\}$ and $\delta\in \{\alpha,\beta,\gamma\}$, vertices in $X^+ \cap S$ cannot resolve a pair of vertices $\langle c_q^{\circ}, c_q^{\star}\rangle$ for any $q\in [m]$.

\smallskip

For all $\delta\in \{\alpha,\beta,\gamma\}$, if $v\in B^{\delta}$, then, for all $X\in \{B^{\delta'}, A^{\delta'}, P^{\delta'},C\}$, $\delta'\in \{\alpha,\beta,\gamma\}$ such that $\delta\neq \delta'$, and $u\in X^+$, we have that $d(u,v)=d(u, \bitrepnullifier(A^{\delta}))+1$. Similarly, for all $\delta\in \{\alpha,\beta,\gamma\}$, if $v\in B^{\delta}$, then, for all $X\in \{A^{\delta}, P^{\delta}\}$ and $u\in X^+$, we have that $d(u,v)=d(u, \bitrepnullifier(A^{\delta}))+1$. Lastly, for each $\langle b_i^{\delta,\circ},  b_i^{\delta,\star}\rangle$, $\delta\in \{\alpha,\beta,\gamma\}$, and $i\in [\sqrt{n}]$, if $X=B^{\delta}$, then, for all $u\in X^+$, either $d(u,b_i^{\delta,\circ})=d(u,b_i^{\delta,\star})=1$, $d(u,b_i^{\delta,\circ})=d(u,b_i^{\delta,\star})=2$, or $d(u,b_i^{\delta,\circ})=d(u,b_i^{\delta,\star})=3$ by the construction in Subsection~\ref{subsubsec:gadget-critical-pairs} and since $\bitrep(X)\setminus \bits(X)$ is a clique. \qedhere
\end{enumerate}
\end{proof}

\begin{lemma}
\label{lemma:3-Part-3-SAT-Met-Dim-forward}
If $\psi$ is a satisfiable \textsc{$3$-Partitioned-$3$-SAT} formula,  then
$G$ admits a resolving set of size $k$.
\end{lemma}
\begin{proof}
Suppose $\pi: X^{\alpha} \cup X^{\beta} \cup X^{\gamma} \mapsto \{\true, \false\}$
is a satisfying assignment for $\psi$.
We construct a resolving set $S$ of size $k$ for $G$ using this assignment.

Initially, set $S = \emptyset$.
For every $\delta \in \{\alpha, \beta, \gamma\}$ and $i \in [\sqrt{n}]$,
consider the assignment $\pi$ restricted to the variables in $X^{\delta}_i$.
By the construction,  there is a vertex in $A^{\delta}_i$ that corresponds
to this assignment.
Include that vertex in $S$.
For each $X \in \{B^{\delta},  A^{\delta},  P^{\delta}, C\}$, where $\delta \in \{\alpha, \beta, \gamma\}$,
we add one vertex from each pair of the false twins in $\bits(X)$ to $S$.
Note that $|S| = k$ and that every vertex in $S$ is distinguished by itself.

In the remaining part of the proof, we show that $S$ is a resolving set of $G$.
First, we prove that all critical pairs are resolved by $S$ in the following claim.

\begin{claim}\label{clm:critpairs}
All critical pairs are resolved by $S$.
\end{claim}
\begin{claimproof}
For each $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$, the critical pair $\langle b^{\delta, \circ}_i, b^{\delta, \star}_i \rangle$
is resolved by the vertex $S\cap A_i^{\delta}$ by the construction.
For each $q\in [m]$, the clause $C_q$ is satisfied by the assignment $\pi$.
Thus, there is a variable $x$ in $C_q$ that satisfies $C_q$ according to $\pi$.
Suppose that $x\in X_i^{\delta}$.
Let $a_{i,\ell}^{\delta}$ be the vertex in $A_i^{\delta}$ corresponding to $\pi$.
Then, by the construction, $d(a_{i,\ell}^{\delta},c_q^{\circ})=2<3=d(a_{i,\ell}^{\delta},c_q^{\star})$.
Thus, every critical pair $\langle c_q^{\circ}, c_q^{\star} \rangle$ is resolved by $S$.
\end{claimproof}

Then, every vertex pair in $V(G)$ is resolved by $S$ by Claim~\ref{clm:critpairs} in conjunction with the second item of the statement of \cref{claim:set-ind}.
%
%To facilitate the rest of the case analysis, let us prove several claims.
%
%Then, we show that every vertex pair inside each part of the graph is resolved by $S$.
%
%\begin{claim}
%For each $X\in \{B^{\delta},A^{\delta},P^{\delta},C\}$, where $\delta\in \{\alpha, \beta, \gamma\}$,
%every pair of distinct vertices in $\bitrep(X)$ is resolved by $S$.
%\end{claim}
%\begin{claimproof}
%The pairs $\langle y_i^a,y_j^b \rangle,$ $\langle y_i^a,y_j^a \rangle$, and $\langle y_i^b,y_j^b \rangle$ $(i,j\in [\lceil \log (|X|+2)\rceil])$ from $\bits(X)$ are resolved by $S\cap \{y_i^a,y_i^b\}$.
%The $i$-th bit vertex $y_i$ and the $j$-th bit vertex $y_j$, where $i,j\in [\lceil \log (|X|+2)\rceil],i\neq j$, are resolved by $S\cap \{y_i^a,y_i^b\}$.
%The pair $\langle y_i^a,y_j \rangle$ and $\langle y_i^b,y_j \rangle$ $(i,j\in [\lceil \log (|X|+2)\rceil])$ are resolved by $S\cap \{y_j^a,y_j^b\}$.
%Thus, every vertex pair in $\bitrep(X)$ is resolved.
%\end{claimproof}
%
%\begin{claim}
%For each $X\in \{B^{\delta},A^{\delta},P^{\delta},C\}$, where $\delta\in \{\alpha, \beta, \gamma\})$,
%every pair of distinct vertices in $X\cup \{\bnull(X)\}$ is resolved by $S$.
%\end{claim}
%\begin{claimproof}
%For each  $\delta\in \{\alpha, \beta, \gamma\}$, every vertex pair in $A^{\delta}\cup \{\bnull(A^{\delta})\}$ is resolved by $\bits(A^{\delta})\cap S$ by our construction.
%Similarly, every vertex pair in $P^{\delta}\cup \{\bnull(P^{\delta})\}$, $\delta\in \{\alpha, \beta, \gamma\}$ is resolved by $\bits(P^{\delta})\cap S$.
%The critical pairs in $C\cup \{\bnull(C)\}$ are resolved by Claim~\ref{clm:critpairs}.
%Moreover, as stated in Subsection~\ref{subsubsec:gadget-critical-pairs}, every pair $\{c^{\circ}_j,  c^{\star}_{\ell}\}$,  $\{c^{\circ}_j,  c^{\circ}_{\ell}\}$,  or
%$\{c^{\star}_j,  c^{\star}_{\ell}\}$ with $j \neq \ell$ is resolved by $\bits(C)\cap S$.
%Thus, every vertex pair in $C\cup \{\bnull(C)\}$ is resolved by $S$.
%Similarly, every vertex pair in $B^{\delta}\cup \{\bnull(B^{\delta})\}$, where $\delta\in \{\alpha, \beta, \gamma\}$ is resolved by $S$.
%\end{claimproof}
%
%\begin{claim}
%For each $X\in \{B^{\delta},A^{\delta},P^{\delta},C\}$, where $\delta\in \{\alpha, \beta, \gamma\}$,
%every vertex pair of $\bitrep(X)\times (V(G)\setminus \bitrep(X))$ is resolved by $S$.
%\end{claim}
%\begin{claimproof}
%For every $v\in \bitrep(X)$ there exists $w\in \bitrep(X)\cap S$, $d(v,\bits(X)\cap S)\leq 2$.
%By the construction, only $X\cup\{\bnull(X)\}$ can be on the distance $2$ from $2$, but this case is covered by \Cref{claim:set-ind}.
%For the rest $u\in V(G)\setminus \bitrep(X)$ the distance is at least $3$. Thus, all pairs $\bitrep(X)\times (V(G)\setminus \bitrep(X))$ are resolved by the selection of such $w$.
%\end{claimproof}
%
%\begin{claim}
%For each $X\in \{B^{\delta},A^{\delta},P^{\delta},C\}$ and $X'\in \{B^{\delta'},A^{\delta'},P^{\delta'}\}$
%such that $\delta,\delta'\in \{\alpha, \beta, \gamma\}$ and $X\neq X'$,
%every vertex pair of $X\times X'$ is resolved by $S$.
%\end{claim}
%\begin{claimproof}
%For every vertex $u\in X$, by the definition of $\bitrep(X)$, $u$ is adjacent to some vertex $y_i\in \bitrep(X)$ that is adjacent to two bit vertices $y^a_i$ and $y^b_i$. Without loss of generality, let $S\cap \{y^a_i,y^b_i\}=y^a_i$. We get that $d(y^a_i,u)=2$, and, for any vertex $v\in X'$, $d(y^a_i,v)\geq 3$ by our construction. Thus, every vertex pair $\langle u,v \rangle$ is resolved by $S$.
%\end{claimproof}
\end{proof}

\begin{lemma}
\label{lemma:3-Part-3-SAT-Met-Dim-backword}
If $G$ admits a resolving set of size $k$, then $\psi$ is a satisfiable \textsc{$3$-Partitioned-$3$-SAT} formula.
\end{lemma}
\begin{proof}
Assume that $G$ admits a resolving set $S$ of size $k$.
First, we prove some properties regarding $S$.
%Recall that, as mentioned in Subsection~\ref{subsubsec:gadget-set},
%there is a pair of false twins for each $y\in\bitrep(X)\setminus \bits(X)$
%for each $X \in \{B^{\delta},  A^{\delta},  P^{\delta}, C\}$ and
%$\delta \in \{\alpha, \beta, \gamma\}$.
%Based on Observation~\ref{obs:twins}, for any resolving set $S$, at least one vertex from each pair of twins is in $S$.
By the first item of the statement of \cref{claim:set-ind}, for each $\delta\in \{\alpha, \beta, \gamma\}$, we have that
\begin{align*}
|S\cap \bits(A^{\delta})| \geq \lceil\log(|A^{\delta}|+2)\rceil + 1,\qquad\, 
 &|S\cap \bits(P^{\delta})| \geq \lceil\log(|P^{\delta}|+2)\rceil + 1, \\
|S\cap \bits(B^{\delta})| \geq \lceil\log(|B^{\delta}|/2+2)\rceil + 1, \quad
&|S\cap \bits(C)| \geq \lceil\log(|C|+2)\rceil + 1.
\end{align*}
Hence, any resolving set $S$ of $G$ already has size at least $$3 \cdot \left(\left(\left\lceil\log(|B^{\alpha}|/2 + 2)\right\rceil + 1\right)
+ \left(\left\lceil\log(|A^{\alpha}|+ 2)\right\rceil + 1\right) + \left(\left\lceil\log(|P^{\alpha}|+ 2)\right\rceil + 1\right) \right) + \lceil\log(|C|+ 2)\rceil + 1.$$

Now, for each $\delta\in\{\alpha, \beta, \gamma\}$ and $i\in[\sqrt{n}]$, consider the critical pair $\langle b_i^{\delta, \circ}, b_i^{\delta, \star} \rangle$.
By the construction mentioned in Subsection~\ref{subsubsec:gadget-critical-pairs}, only $v\in A_i^{\delta}\cup \{b_i^{\delta, \circ}, b_i^{\delta, \star}\}$ resolves a pair $\langle b_i^{\delta, \circ}, b_i^{\delta, \star} \rangle$.
Indeed, for all $X \in \{B^{\delta'},  A^{\delta'},  P^{\delta'}, C\}$ and $\delta' \in \{\alpha, \beta, \gamma\}$, no vertex in $X^+$ can resolve such a pair by the third item of the statement of \cref{claim:set-ind}. Also, for all $X\in \{A^{\delta''},P^{\delta'},C\}$, $\delta' \in \{\alpha, \beta, \gamma\}$, $\delta'' \in \{\alpha, \beta, \gamma\}$ such that $\delta\neq \delta''$, and $u\in X$, we have that $d(u,b_i^{\delta, \circ})=d(u,b_i^{\delta, \star})=d(u,\bitrepnullifier(A^{\delta}))+1$. Furthermore, for any $a\in A_j^{\delta}$ with $j\in [\sqrt{n}]$ such that $i\neq j$, we have that $d(a,b_i^{\delta, \circ})=d(a,b_i^{\delta, \star})=2$ by construction and since $B^{\delta}$ is a clique. 
Hence, since any resolving set $S$ of $G$ of size at most $k$ can only admit at most another $3\sqrt{n}$ vertices, we get that equality must in fact hold in every one of the aforementioned inequalities, and any resolving set $S$ of $G$ of size at most $k$ contains one vertex from $A_i^{\delta}\cup \{b_i^{\delta, \circ}, b_i^{\delta, \star}\}$ for all $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$. Hence, any resolving set $S$ of $G$ of size at most $k$ is actually of size exactly $k$.

Next, for each $\delta\in \{\alpha, \beta, \gamma\}$, we construct an assignment $\pi: X^{\alpha} \cup X^{\beta} \cup X^{\gamma} \mapsto \{\true, \false\}$ in the following way.
If $a_{i,\ell}^{\delta}\in S$ and $\pi':X_{i}^{\delta}\rightarrow \{\true, \false\}$ corresponds to the underlying assignment of $a_{i,\ell}^{\delta}$ for the variables in $X_{i}^{\delta}$,
then let $\pi:X_{i}^{\delta}\rightarrow \{\true, \false\}:=\pi'$ for each $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$.
If $S\cap A_i^{\delta}=\emptyset$, then one of $ b_i^{\delta, \circ}, b_i^{\delta, \star}$ is in $S$, and we can use an arbitrary assignment of the variables in the bucket $X_i^{\delta}$.

We contend that the constructed assignment $\pi$ satisfies every clause in $C$.
Since $S$ is a resolving set, it follows that, for every clause $c_q\in C$,
there exists $v\in S$ such that $d(v, c_q^{\circ})\neq d(v, c_q^{\star})$.
Notice that, for any $v$ in $\bits(A^{\delta}), \bits(B^{\delta}), \bits(P^{\delta})$ for any $\delta\in \{\alpha, \beta, \gamma\}$ or in $\bits(C)$, we have $d(v, c_q^{\circ})= d(v, c_q^{\star})$ by the third item of the statement of Lemma~\ref{claim:set-ind}.
Further, for any $v\in B^{\delta}$ and any $\delta\in \{\alpha, \beta, \gamma\}$, we have that $d(v, c_q^{\circ})=d(v, c_q^{\star})=d(v,\bitrepnullifier(P^{\delta}))+1$.
Thus, $v\in S\cap \bigcup\limits_{\delta\in \{\alpha, \beta, \gamma\}} A^{\delta}$.
Without loss of generality, suppose that $c_q^{\circ}$ and $c_q^{\star}$ are resolved by
$a_{i,\ell}^{\alpha}$.
So, $d(a_{i,\ell}^{\alpha}, c_q^{\circ}) \neq d(a_{i,\ell}^{\alpha}, c_q^{\star})$.
By the construction, the only case where $d(a_{i,\ell}^{\alpha}, c_q^{\circ}) \neq d(a_{i,\ell}^{\alpha}, c_q^{\star})$ is when
$C_q$ contains a variable $x\in X_i^{\alpha}$ and $\pi(x)$ satisfies $C_q$.
Thus, we get that the clause $C_q$ is satisfied by the assignment $\pi$.
%Then, the shortest path from $a_{i,l}^{\alpha}$ to $c_q^{\circ}$ passes through the only vertex $w\in P_T^{\alpha}\cup P_F^{\alpha}$ that is in the neighborhood of $c_i^{\circ}$ and not in the neighborhood of $c_q^{\circ}$.
%Thus $d(a_{i,l}^{\alpha}, c_q^{\circ})=2$.
%See, that the neighborhoods of $c_i^{\circ}$ and $c_i^{\star}$ differ by only one vertex, since we have a valid \textsc{3P-3SAT} instance.
%Since $d(a_{i,l}^{\alpha}, c_q^{\star})>2$ by the construction,
%the only way to get shorter path from $a_{i,l}^{\alpha}$ to $c_i^{\circ}$ is through $w\in P_T^{\alpha}\cup P_F^{\alpha}$ with the distance $2$.
%But this path exists in the construction, if the underlying assignment of $a_{i,l}^{\alpha}$ for variables $B_{i}^{\alpha}$ assign the same value which satisfies the clause $c_j$.

Since $S$ resolves all pairs $\langle c_q^{\circ},c_q^{\star}\rangle$ in $V(G)$, then the assignment $\pi$ constructed above indeed satisfies every clause $c_q$, completing the proof.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:reduction-3-SAT-Met-Dim-VC}.] 
As mentioned before, by \cref{prop:3-SAT-to-3-Partition-3-SAT}, there is a polynomial-time reduction from \textsc{3-SAT} to \textsc{$3$-Partitioned-$3$-SAT} that increases the number of variables and clauses by a constant factor.
In Subsection~\ref{subsec:reduction-3-Par-3-SAT-Met-Dim}, we presented a reduction that takes an instance $\psi$ of \textsc{$3$-Partitioned-$3$-SAT} and returns an equivalent instance $(G,k)$ of \textsc{Metric Dimension} (by Lemmas~\ref{lemma:3-Part-3-SAT-Met-Dim-forward} and \ref{lemma:3-Part-3-SAT-Met-Dim-backword}) in $2^{\OO(\sqrt{n})}$ time. 
Note that $V(G)=2^{\OO(\sqrt{n})}$. 
%Then, note that the diameter of the graph $G$ is $4$.
Further, note that taking all the vertices in $B^{\delta}$, $P^{\delta}$, and $\bitrep(X)$ for all $X \in \{B^{\delta},  A^{\delta},  P^{\delta}, C\}$ and $\delta \in \{\alpha, \beta, \gamma\}$, results in a vertex cover of $G$. Hence, 
\begin{equation*}
\begin{split}
\vc(G) &\leq 3 \cdot \left(\left(\left\lceil\log(|B^{\alpha}|/2 + 2)\right\rceil + 1\right)
+ \left(\left\lceil\log(|A^{\alpha}|+ 2)\right\rceil + 1\right) + \left(\left\lceil\log(|P^{\alpha}|+ 2)\right\rceil + 1\right)\right) +
\\
& 3\cdot (|B^{\alpha}|+|P^{\alpha}|) +  (\lceil\log(|C|+ 2)\rceil + 1)=\OO(\sqrt{n}).
\end{split}
\end{equation*}
Lastly, the metric dimension of $G$ is at most 
\begin{equation*}
\begin{split}
k &= 3 \cdot \left(\sqrt{n} + \left(\left\lceil\log(|B^{\alpha}|/2 + 2)\right\rceil + 1\right)
+ \left(\left\lceil\log(|A^{\alpha}|+ 2)\right\rceil + 1\right) + \left(\left\lceil\log(|P^{\alpha}|+ 2)\right\rceil + 1\right) \right) +
\\
&  (\lceil\log(|C|+ 2)\rceil + 1)=\OO(\sqrt{n}).
\end{split}
\end{equation*}
Thus, $\vc(G)+k=\OO(\sqrt{n})$.
\end{proof}


==> vc_lower_bound-GS.tex <==
\section{\gsfull: Lower Bounds Regarding Vertex Cover}
\label{sec:lower-bound-vertex-cover-GS}

In this section, we follow the same
template as in Section~\ref{sec:lower-bound-vertex-cover} and first prove
the following theorem.

\begin{theorem}
\label{thm:reduction-3-SAT-GS-VC}
There is an algorithm that, given an instance
$\psi$ of \textsc{3-Partitioned-3-SAT} on $N$ variables,  
runs in time $2^{\calO(\sqrt{N})}$, and constructs an equivalent 
instance $(G, k)$ of \gsfull such that 
$\vc(G) + k = \OO(\sqrt{N})$ (and $|V(G)| = 2^{\OO(\sqrt{N})}$).
\end{theorem}

The proofs of the following two
corollaries are analogous to the ones in the previous section.

\begin{corollary}
\label{cor:GS-vc-lower-bound-algo}
Unless the \ETH\ fails, 
\gsfull does not admit an algorithm 
running in time $2^{o(\vc^2)} \cdot n^{\OO(1)}$. 
\end{corollary}
\begin{corollary}
\label{cor:GS-vc-lower-bound-kernel}
Unless the \ETH\ fails, 
\gsfull\ does not admit a kernelization algorithm that
reduces the solution size $k$ and
outputs a kernel with $2^{o(k + \vc)}$ vertices. 
\end{corollary}


\subsection{Reduction}
\label{subsec:reduction-3-Par-3-SAT-Geod-Set}

Consider an instance $\psi$ of \textsc{3-Partitioned-3-SAT}
with $X^{\alpha}, X^{\beta}, X^{\gamma}$ the partition of the variable set, where $|X^{\alpha}| = |X^{\beta}| = |X^{\gamma}|=n$. 
By adding dummy variables in each of these sets, we can assume that $\sqrt{n}$ is an integer.
Further, let $\calC=\{C_1, \dots, C_m\}$ be the set of all the clauses of $\psi$.
From $\psi$, we construct the graph $G$ as follows.
We describe the first part of the construction for $X^{\alpha}$, with the constructions for $X^{\beta}$ and $X^{\gamma}$ being analogous.
We rename the variables in $X^{\alpha}$
to $x^{\alpha}_{i, j}$ for $i, j \in [\sqrt{n}]$.

\begin{figure}[H]
    \centering
        \includegraphics[scale=1.25]{./images/reduction-vc.pdf}
    \caption{Overview of the reduction.
    Sets with elliptical boundaries are independent sets, and sets with rectangular boundaries are cliques.
    For each $\delta \in \{\alpha, \beta, \gamma\}$, the sets $V^{\delta}$ and $U$ almost form a complete bipartite graph modulo the matching (marked by dotted edges), which is excluded.
    Yellow lines from a vertex to a set denote that this vertex is connected to all the vertices in that set.
    The green and red lines across the $A_i^{\alpha}$ and $T^{\alpha}\cup F^{\alpha}$ transfer, in some sense, for each $w\in A_i^{\alpha}$, the underlying assignment structure.
    If an underlying assignment $w$ sets the $j^{th}$ variable to \true, then we add the green edge $(w,t_{j}^{\alpha})$, and otherwise, we add the red edge $(w,f_{j}^{\alpha})$.
    For all $q \in [m]$ and $\delta \in \{\alpha, \beta, \gamma\}$, let $x_{i, j}^{\delta}$ be the variable in $X^{\delta}$ that is contained in the clause $C_q$ in $\psi$. So, for all $q\in [m]$, if assigning \true\ (\false, respectively) to $x_{i, j}^{\delta}$ satisfies $C_q$, then we add the edge $(c_q,t_j^{\delta})$ ($(c_q,f_j^{\delta})$, respectively).}
    \label{fig:reduction-vc}
\end{figure}


\begin{itemize}
\item We partition the variables of $X^{\alpha}$ into \emph{buckets}
$X^{\alpha}_1,  X^{\alpha}_2,  \dots , X^{\alpha}_{\sqrt{n}}$
such that each bucket contains $\sqrt{n}$ many variables.
Let $X^{\alpha}_i = \{x^{\alpha}_{i, j}\ |\ j \in [\sqrt{n}]\}$ for all $i \in [\sqrt{n}]$.

\item For every bucket $X^{\alpha}_i$, we add an independent set $A^{\alpha}_i$ of $2^{\sqrt{n}}$ new vertices, and we add two isolated edges $(a^{\alpha}_{i, 1},b^{\alpha}_{i, 1})$ and $(a^{\alpha}_{i, 2},b^{\alpha}_{i, 2})$. Let $B^{\alpha}=\{a^{\alpha}_{i, j},b^{\alpha}_{i, j} \mid i\in [\sqrt{n}],j\in \{1,2\}\}$.
For all $i \in [\sqrt{n}]$ and $u \in A_i^{\alpha}$, we make both $a^{\alpha}_{i,1}$ and $a^{\alpha}_{i,2}$ adjacent to $u$ (see \cref{fig:reduction-vc}).

Each vertex in $A^{\alpha}_i$ corresponds to a certain possible assignment of
variables in $X^{\alpha}_i$. 
\item Then, we add three independent sets $T^{\alpha}$, $F^{\alpha}$, and $V^{\alpha}$ on $\sqrt{n}$ vertices each: $T^{\alpha}=\{t^{\alpha}_i \mid i\in [\sqrt{n}]\}$, $F^{\alpha}=\{f^{\alpha}_i \mid i\in [\sqrt{n}]\}$, and $V^{\alpha}=\{v^{\alpha}_i \mid i\in [\sqrt{n}]\}$. 
\item For each $i\in [\sqrt{n}]$, we connect $v^{\alpha}_i$ with all the vertices in $A^{\alpha}_i$.
\item For each $i\in [\sqrt{n}]$, we add a special vertex $g^{\alpha}_i$ (also referred to as a $g$-vertex later on) that is adjacent to each vertex in $T^{\alpha}\cup F^{\alpha}$. Further, $g^{\alpha}_i$ is also adjacent to both $a^{\alpha}_{i, 1}$ and $a^{\alpha}_{i, 2}$ (see \cref{fig:reduction-vc}).
\end{itemize}
This finishes the first part of the construction. 
The second step is to connect the three previously constructed parts for $X^{\alpha}$, $X^{\beta}$, and $X^{\gamma}$.
\begin{itemize}
\item We introduce a vertex set $U=\{u_i \mid i\in [\sqrt{n}]\}$ that forms a clique. Then, for each $u_i$, we add an edge to a new vertex $u'_i$.
Thus, we have a matching $\{(u_i,u'_i) \mid i\in [\sqrt{n}]\}$.
Let $U'=\{u'_i\mid i\in [\sqrt{n}]\}$.
\item For each $\delta\in \{\alpha, \beta, \gamma\}$, we make it so that the vertices of $U\cup V^{\delta}$ form almost a complete bipartite graph, i.e., $E(G)$ contains edges between all pairs $\langle v,w \rangle$ where $v\in U$ and $w\in V^{\delta}$, except for the matching $\{(v^{\delta}_i,u_i) \mid i\in [\sqrt{n}]\}$.
\item For each $\delta\in \{\alpha, \beta, \gamma\}$ and $i\in [\sqrt{n}]$, we make $g_i^{\delta}$ adjacent to each vertex in $U$.
\item For each $C_q\in \calC$, we add a new vertex $c_q$. Let $C=\{c_q \mid q\in [m]\}$. 
Since we are considering an instance of \PSAT, for each $\delta\in \{\alpha, \beta, \gamma\}$, there is exactly one variable in $C_q$ that lies in $X^{\delta}_i$, and, without loss of generality, let it be $x_{i,j}^{\delta}$. 
Then, we make $c_q$ adjacent to $u_{i}$. 
Finally, if $x_{i,j}^{\delta}=\true$ ($x_{i,j}^{\delta}=\false$, respectively) satisfies $C_q$, then $(c_q,t^{\delta}_j)\in E(G)$ ($(c_q,f^{\delta}_j)\in E(G)$, respectively).
\end{itemize}

This concludes the construction of $G$.
The reduction returns $(G,  k)$
as an instance of \textsc{Geodetic Set} where $k = 10\sqrt{n}$.

\subsection{Correctness of the Reduction}

Suppose, given an instance $\psi$ of \textsc{$3$-Partitioned-$3$-SAT}, that the reduction above returns $(G, k)$ as an instance of \textsc{Geodetic Set}. We first prove the following lemmas which will be helpful in proving the correctness of the reduction, and note that we use distances between vertices to prove that certain vertices are not contained in shortest paths.

\begin{lemma}\label{lem:S'crit}
For all $\delta,\delta'\in \{\alpha, \beta, \gamma\}$, the shortest paths between any two vertices in $B^{\delta}\cup U\cup U'$ do not cover any vertices in $C$ nor $V^{\delta''}$.
\end{lemma}

\begin{proof}
Since, for all $i\in [\sqrt{n}]$, $j\in \{1,2\}$, and $\delta\in \{\alpha, \beta, \gamma\}$, the shortest path from $b_{i, j}^{\delta}$ ($u'_i$, respectively) to any other vertex in $G$ first passes through $a_{i, j}^{\delta}$ ($u_i$, respectively), it suffices to prove the statement of the lemma for the shortest paths between any two vertices in $U\cup (B^{\delta}\setminus \{b_{i,j}^{\delta} \mid i\in [\sqrt{n}],j\in \{1,2\}\})$. 

For all $i\in [\sqrt{n}]$, $j\in \{1,2\}$, and $\delta,\delta'\in \{\alpha, \beta, \gamma\}$, we have $d(a_{i, 1}^{\delta},a_{i, 2}^{\delta})=2$ and $d(a_{i, j}^{\delta},w)\geq 2$ for all $w\in V^{\delta'}\cup C$. For all $i,i'\in [\sqrt{n}]$, $j,j'\in \{1,2\}$, and $\delta,\delta',\delta''\in \{\alpha, \beta, \gamma\}$ such that $i\neq i'$ and/or $\delta\neq \delta'$ (i.e., we are not in the previous case), we have $d(a_{i, j}^{\delta},a_{i', j'}^{\delta'})=4$, $d(a_{i, j}^{\delta},w)=d(a_{i', j'}^{\delta'},w)=3$ for all $w\in C$, and, for any $w'\in V^{\delta''}$, we have $d(a_{i, j}^{\delta},w')\geq 2$, $d(a_{i', j'}^{\delta'},w')\geq 2$, and $3\in \{d(a_{i, j}^{\delta},w'),d(a_{i', j'}^{\delta'},w')\}$.
Further, for any $i, i'\in [\sqrt{n}]$ with $i\neq i'$, $d(u_i,u_{i'})=1$.
Lastly, for all $i, i'\in [\sqrt{n}]$, $j\in \{1,2\}$, and $\delta,\delta'\in \{\alpha, \beta, \gamma\}$, we have $d(a_{i,j}^{\delta},u_{i'})=2$, while $d(a_{i,j}^{\delta},w)\geq 2$ for all $w\in V^{\delta'}\cup C$. Hence, the vertices in $C$ and $V^{\delta'}$ are not covered by any shortest path between any of these pairs.
\end{proof}

\begin{lemma}\label{lem:forceA}
For all $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$, $v_i^{\delta}$ can only be covered by a shortest path from a vertex in $A_i^{\delta} \cup \{v_i^{\delta}\}$ to another vertex in $G$.
\end{lemma}

\begin{proof}
As stated in the proof of \cref{lem:S'crit}, we do not need to consider any shortest path with an endpoint that is a degree-$1$ vertex.
First, we show that $v_i^{\delta}$ cannot be covered by a shortest path with one endpoint in $U$ and the other not in $A_i^{\delta} \cup \{v_i^{\delta}\}$. To cover this case, by \cref{lem:S'crit}, we just need to consider all shortest paths between a vertex $w\in U$ and any other vertex $z\in V(G)\setminus (U\cup U'\cup B^{\alpha} \cup B^{\beta} \cup B^{\gamma} \cup A_i^{\delta} \cup \{v_i^{\delta}\})$.
Note that $d(z,v_i^{\delta})\geq 2)$, and so, if $d(w,z)\leq 2$, then $v_i^{\delta}$ is not covered by the pair $\langle w,z \rangle$.
Further, $d(w,w')\leq 3$ for all $w'\in V(G)$, and, for all $z'\in V(G)$ such that $d(w,z')=3$, we have that $d(z',v_i^{\delta})\geq 3$.
Hence, $v_i^{\delta}$ cannot be covered by a shortest path with one endpoint in $U$ and the other not in $A_i^{\delta} \cup \{v_i^{\delta}\}$.

For all $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$, we have that $N(v_i^{\delta})=A^{\alpha}_i\cup (U\setminus \{u_i\})$, and $d(w,z)\leq 2$ for any $w,z\in N(v_i^{\delta})$. Hence, for a shortest path between two vertices in $V(G)\setminus (A_i^{\delta} \cup \{v_i^{\delta}\})$ to contain $v_i^{\delta}$, that path must also contain two vertices from $N(v_i^{\delta})$. Furthermore, since $v_i^{\delta}$ cannot be covered by a shortest path with one endpoint in $U$ and the other not in $A_i^{\delta} \cup \{v_i^{\delta}\}$, any shortest path whose endpoints are in $V(G)\setminus (A_i^{\delta} \cup \{v_i^{\delta})\}$ that could cover $v_i^{\delta}$ cannot have any of its endpoints in $N(v_i^{\delta})$, and thus, must have length at least $4$. In particular, this proves the following property that we put as a claim to make reference to later.

\begin{claim}\label{clm:neighbors-v}
For any shortest path whose endpoints cannot be in $N[v_i^{\delta}]$, if its first and second endpoints are at distance at least $\ell_1$ and $\ell_2$, respectively, from any vertex in $N(v_i^{\delta})$, then this shortest path cannot cover $v_i^{\delta}$ if it has length less than $\ell_1+\ell_2+2$.
\end{claim} 

We finish with a case analysis of the possible pairs $\langle u,v \rangle$ to prove that no such shortest path covering $v_i^{\delta}$ exists using \cref{clm:neighbors-v}. We note that, by the arguments above, we do not need to consider the case where $u$ and/or $v$ is a degree-$1$ vertex, nor the case where both $u$ and $v$ are in $U\cup B^{\alpha} \cup B^{\beta} \cup B^{\gamma}$, nor the case where one of $u$ and $v$ is in $U$. We now proceed with the case analysis assuming that $u,v\notin N[v_i^{\delta}]$.

\begin{itemize}
\item \textbf{Case 1:} $\boldsymbol{u\in A_{i'}^{\delta'}}$ \textbf{for any} $\mathbf{i'\in [\sqrt{n}]}$ \textbf{and} $\boldsymbol{\delta'\in \{\alpha, \beta, \gamma\}}$ \textbf{such that} $\boldsymbol{A_{i'}^{\delta'}\neq A_{i}^{\delta}}$\textbf{.}
First, $u$ is at distance at least $2$ from any vertex in $N(v_i^{\delta})$, and hence, if $d(u,v)\leq 4$, then we are done by \cref{clm:neighbors-v}. Note that $d(u,v)\leq 4$ as long as $v\notin A_{i'}^{\delta''}$ for any $\delta''\in \{\alpha, \beta, \gamma\}$ such that $\delta''\neq \delta'$, since $u$ is at distance $2$ from every vertex in $U\setminus \{u_{i'}\}$. However, in the case where $v\in A_{i'}^{\delta''}$, we have that $v$ is also at distance at least $2$ from any vertex in $N(v_i^{\delta})$, and so, since $d(u,v)\leq 5$, we are done by \cref{clm:neighbors-v}.

\item \textbf{Case 2:} $\mathbf{u\in C}$ \textbf{or} $\mathbf{u}$ \textbf{is a} $\mathbf{g}$\textbf{-vertex.}
By \cref{clm:neighbors-v} and the previous case, it suffices to note that $d(u,v)\leq 3$ as long as $v\notin A_{i'}^{\delta'}$ for any $i'\in [\sqrt{n}]$ and $\delta'\in \{\alpha, \beta, \gamma\}$.

\item \textbf{Case 3:} $\boldsymbol{u\in T^{\delta'}\cup F^{\delta'}}$ \textbf{for any} $\boldsymbol{\delta'\in \{\alpha, \beta, \gamma\}}$ \textbf{such that} $\mathbf{\boldsymbol{\delta}'\neq \boldsymbol{\delta}}$\textbf{.}
Since $u$ is at distance $2$ from any vertex in $U$, we have that $d(u,v)\leq 4$, and we are done by \cref{clm:neighbors-v}.

\item \textbf{Case 4:} $\boldsymbol{u\in T^{\delta}\cup F^{\delta}}$\textbf{.}
First, if $v\notin A_{i'}^{\delta'}$ for any $i'\in [\sqrt{n}]$ and $\delta'\in \{\alpha, \beta, \gamma\}$, and $v$ is a vertex with a superscript $\delta$, then $d(u,v)\leq 3$. Otherwise, the path from $u$ to $v$ contains a vertex in $U\cup C$, and thus, does not cover $v_i^{\delta}$ since $d(u,v_i^{\delta})\geq 2$, $u$ is at distance~$2$ (at most $3$, respectively) from any vertex in $U$ ($C$, respectively), and $v_i^{\delta}$ is at distance at least~$2$ from any vertex in $C$. Thus, we are done by the previous cases and \cref{clm:neighbors-v}.

\item \textbf{Case 5:} $\boldsymbol{u\in V^{\delta'}}$ \textbf{for any} $\boldsymbol{\delta'\in \{\alpha, \beta, \gamma\}}$\textbf{.}
For any $\delta''\in \{\alpha, \beta, \gamma\}$, if $v\in B^{\delta''}\cup V^{\delta''}$, then $d(u,v)\leq 3$, and we are done by the previous cases and \cref{clm:neighbors-v}. \qedhere
\end{itemize}
\end{proof}

\begin{lemma}\label{lem:GS-vc-forward}
If $G$ admits a geodetic set of size $k$, then $\psi$ is a satisfiable \textsc{$3$-Partitioned-$3$-SAT} formula.
\end{lemma}

\begin{proof}
Assume that $G$ admits a geodetic set $S$ of size $k$.
Then, let us consider the set $S'=\{u_i'\mid i\in [\sqrt{n}]\}\cup \{b^{\delta}_{i,1}, b^{\delta}_{i,2}\mid \delta\in \{\alpha, \beta, \gamma\}, i\in [\sqrt{n}]\}$ of all the degree-1 vertices in $G$.
By \cref{obs:pendant}, $S'\subseteq S$. By \cref{lem:forceA}, for each $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$, there is at least one vertex from $A_i^{\delta}\cup \{v_i^{\delta}\}$ in $S$.
Since $|S'|=7\sqrt{n}$ and $k=10\sqrt{n}$, for each $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$, $S$ contains exactly $1$ vertex from $A_i^{\delta}\cup \{v_i^{\delta}\}$.

By \cref{lem:S'crit}, the shortest paths between vertices in $S'$ do not cover vertices in $C$, and thus, the $3\sqrt{n}$ vertices in $S\setminus S'$ must cover them.

For this goal, the vertices in $S$ that are in $V^{\delta}$ for any $\delta\in \{\alpha, \beta, \gamma\}$ are irrelevant. Indeed, any such vertex is at distance at most~$3$ from any other vertex in $S\setminus S'$, while every vertex in $S\setminus S'$ is at distance at least~$2$ from any vertex in $C$.
So, let us consider one vertex from $A^{\delta}$ for some $\delta\in \{\alpha, \beta, \gamma\}$ that lies in $S$, say, without loss of generality, $w\in A_i^{\alpha}$.
Note that $d(w,u'_i)=4$ and recall that $u'_i\in S$.
For any $q\in [m]$, there is a path of length $4$ between $w$ and $u'_i$ that covers $c_q$ if there is $v\in T^{\alpha}\cup F^{\alpha}$ such that both $(w,v)$ and $(v,c_q)$ are in $E(G)$.
But, by the construction, such an edge $(w,v)\in E(G)$ corresponds to an assignment of a variable that occurs in $c_q$, i.e., $(v,c_q)\in E(G)$ if the corresponding assignment to $v$ (\true\ or \false) satisfies the clause $C_q$ of the instance $\psi$.
Since $S$ is a geodetic set, for each $q\in[m]$, there is a vertex $w\in \bigcup_{\delta\in \{\alpha, \beta, \gamma\}}A^{\delta} \cap S$ that covers $c_q$ by a shortest path to some $u\in U'$.
Thus, let $\pi: X^{\alpha}\cup X^{\beta} \cup X^{\gamma} \rightarrow \{\true, \false\}$ be the retrieved assignment from the partial assignments that correspond to such vertices $w$ that are in both $S$ and $\bigcup_{\delta\in \{\alpha, \beta, \gamma\}}A^{\delta}$, and that is completed by selecting an arbitrary assignment for the variables in the buckets $X_i^{\delta}$ where $A_{i}^{\alpha}\cap S=\emptyset$.

Finally, as we observed above, for each $q\in[m]$, $c_q$ is covered, and thus, the constructed assignment $\pi$ satisfies all the clauses in $\calC$.
\end{proof}

\begin{lemma}\label{lem:GS-vc-backward}
If $\psi$ is a satisfiable \textsc{$3$-Partitioned-$3$-SAT} formula,  then
$G$ admits a geodetic set of size $k$.
\end{lemma}
\begin{proof}
Suppose $\pi: X^{\alpha}\cup X^{\beta} \cup X^{\gamma} \rightarrow \{\true, \false\}$ is a satisfying assignment for $\psi$.
We construct a geodetic set $S$ of size $k$ for $G$ using this assignment. 
Initially, let $$S=\{u_i'\mid i\in [\sqrt{n}]\}\cup \{b^{\delta}_{i,1}, b^{\delta}_{i,2}\mid \delta\in \{\alpha, \beta, \gamma\}, i\in [\sqrt{n}]\}.$$
At this point, $|S|=7\sqrt{n}$. 
Now, for each $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$, we add one vertex from $A^{\delta}_i$ to $S$ in the following way. 
For the bucket of variables $X^{\delta}_i$, consider how the variables of $X^{\delta}_i$ are assigned by $\pi$, and denote this assignment restricted to $X^{\delta}_i$ by $\pi^{\delta}_i$. 
Since $A^{\delta}_i$ contains a vertex for each of the possible $2^{\sqrt{n}}$ assignments and each of those corresponds to a certain assignment of $X^{\delta}_i$, we will find $w\in A^{\delta}_i$ that matches the assignment $\pi^{\delta}_i$. 
Then, we include this $w$ in $S$ as well. 
At the end, $|S|=10\sqrt{n}$.

Now, we show that $S$ is indeed a geodetic set of $G$.
First, recall that the vertices of $S$ are covered by any shortest path between them and any another vertex in $S$.
Further, recall that the neighbors of the degree-$1$ vertices in $S$ are also covered by the shortest paths between their degree-$1$ neighbor in $S$ and any another vertex in $S$. 
In the following case analysis, we omit the cases just described above. In each case, we consider sets of vertices that we want to cover by shortest paths between pairs of vertices in $S$. 

\begin{itemize}
\item {\bf Case 1:} $\boldsymbol{A_i^{\delta}\cup \{g_i^{\delta}\} \mid i\in [\sqrt{n}], \delta\in \{\alpha, \beta, \gamma\}\}}$\textbf{.}
For each $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$, there is a shortest path of length~$4$ between $b_{i, 1}^{\delta}$ and $b_{i, 2}^{\delta}$ that contains $g_i^{\delta}$ (any vertex in $A_i^{\delta}$, respectively).

\item {\bf Case 2:} $\boldsymbol{T^{\delta}\cup F^{\delta}}$ \textbf{for any} $\boldsymbol{\delta\in \{\alpha, \beta, \gamma\}}$\textbf{.}
For each $\delta\in \{\alpha, \beta, \gamma\}$ and $i,i'\in [\sqrt{n}]$ such that $i\neq i'$, there is a shortest path of length~$6$ between $b_{i, 1}^{\delta}$ and $b_{i', 1}^{\delta}$ that is as follows.
First, it goes to $a_{i, 1}^{\delta}$ and then through $g^{\delta}_i$ to $w\in T^{\delta}\cup F^{\delta}$, and then through $g_{i'}^{\delta}$ to $a_{i', 1}^{\delta}$, before finishing at $b_{i', 1}^{\delta}$.
Since, for each $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$, $g_i^{\delta}$ is adjacent to all the vertices in $T^{\delta}\cup F^{\delta}$, the described path of length $6$ covers $T^{\delta}\cup F^{\delta}$.

\item {\bf Case 3:} $\boldsymbol{\{c_q\}_{q\in [m]}}$ \textbf{and} $\boldsymbol{V^{\delta}}$ \textbf{for any} $\boldsymbol{\delta\in \{\alpha, \beta, \gamma\}}$\textbf{.} 
For all $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$, consider the vertex $w\in A_i^{\delta}\cap S$. Recall that this $w$ corresponds to the assignment $\pi_i^{\delta}$, i.e., $\pi$ that is restricted to the subset of variables $X_i^{\delta}$.
First, there is a shortest path of length~$4$ between $w$ and $u'_i$ that contains $v_i^{\delta}$, $u_{i'}$ (for some $i'\in [\sqrt{n}]$ such that $i\neq i'$), and $u_i$.
Second, for each $q\in [m]$, there exists $i\in [\sqrt{n}]$ and $\delta\in \{\alpha, \beta, \gamma\}$ such that there is a shortest path of length $4$ from $w\in A_{i}^{\delta}$ to $u'_i$ that covers $c_q$.
Consider the variable that satisfied the clause $C_q$ of the initial instance $\psi$ under the assignment $\pi$, and, without loss of generality, let it be $x_{i, j}^{\delta}$.
Then, consider the bucket $A_i^{\delta}$ and select $w\in A_i^{\delta}$ such that $w$ corresponds to $\pi_i^{\delta}$.
Since $w$ corresponds to $\pi_i^{\delta}$, if $\pi(x^{\delta}_{i, j})=\true$ ($\pi(x^{\delta}_{i, j})=\false$, respectively), then $(w,t^{\delta}_j)\in E(G)$ ($(w,f^{\delta}_j)\in E(G)$, respectively) and, since $x_{i, j}^{\delta}=\true$ ($x_{i, j}^{\delta}=\false$, respectively) satisfies $C_q$, $(t^{\delta}_{j},c_q)\in E(G)$ ($(f^{\delta}_{j},c_q)\in E(G)$, respectively) as well.
Thus, we have a shortest path of length~$4$ that goes from $w$ to $t^{\delta}_j$ ($f^{\delta}_j$ in the latter case) to $c_q$ to $u_i$ to $u_i'$.
This way, all the vertices in $\{c_q\mid q\in [m]\}$ are also covered.
\end{itemize}

This covers all the vertices in $V(G)$, and thus, $S$ is a geodetic set of $G$.
\end{proof}

\begin{proof}[Proof of \Cref{thm:reduction-3-SAT-GS-VC}.] 
As mentioned before, by \Cref{prop:3-SAT-to-3-Partition-3-SAT}, there is a polynomial-time reduction from \textsc{3-SAT} to \textsc{$3$-Partitioned-$3$-SAT} that increases the number of variables and clauses by a constant factor.
In \cref{subsec:reduction-3-Par-3-SAT-Geod-Set}, we presented a reduction that takes an instance $\psi$ of \textsc{$3$-Partitioned-$3$-SAT} and returns an equivalent instance $(G,k)$ of \textsc{Geodetic Set} (by Lemmas~\ref{lem:GS-vc-forward} and \ref{lem:GS-vc-backward}) in $2^{\OO(\sqrt{n})}$ time. 
Note that $V(G)=2^{\OO(\sqrt{n})}$. 
Further, note that taking all the vertices in $B^{\delta}$, $V^{\delta}$, $T^{\delta}$, $F^{\delta}$, $U$, $C$, and $g^{\delta}_i$ for all $i\in [\sqrt{n}]$ and $\delta \in \{\alpha, \beta, \gamma\}$, results in a vertex cover of $G$. Hence, 

$$\vc(G) \leq 3 \cdot (|B^{\alpha}| + |V^{\alpha}| + |T^{\alpha}| + |F^{\alpha}| + \sqrt{n}) + |U| + |C|=\OO(\sqrt{n}).$$

Lastly, any minimum-size geodetic set of $G$ has size at most $k=10\sqrt{n}$.
Thus, $\vc(G)+k=\OO(\sqrt{n})$.
\end{proof}
